Moduli Problems in Abelian Categories and the Reconstruction Theorem

We give a moduli-theoretic proof of the classical theorem of Gabriel, stating that a scheme can be reconstructed from the abelian category of quasi-coherent sheaves over it. The methods employed are elementary and allow us to extend the theorem to (quasi-compact and separated) algebraic spaces. Using more advanced technology (and assuming flatness) we also give a proof of the folklore result that the group of autoequivalences of the category of quasi-coherent sheaves consists of automorphisms of the underlying space and twists by line bundles. We apply our strategy to prove analogous statements for categories of sheaves twisted by a Gm-gerbe. Our methods allow us to treat even gerbes not coming from a Brauer class. As a pleasant consequence, we deduce a Morita theory for sheaves of abelian categories.

==> comments.tex <==
\section*{Comments} % (fold)
\label{sec:comments}
 \makeatletter
 \providecommand\@dotsep{5}
 \makeatother
 \listoftodos\relax

\todo[inline]{remove comments!}

Gabriel was IV.3
Rosenberg Proposition 10.7.1
Lurie Remark 5.12


this is how you cite the stacks project

\cite[\href{http://stacks.math.columbia.edu/tag/00NZ}{Tag 00NZ}]{stacks-project}

bibtex for the stacks project

@misc{stacks-project, 
  author       = {The {Stacks Project Authors}}, 
  title        = {\itshape Stacks Project}, 
  howpublished = {\url{http://stacks.math.columbia.edu}}, 
  year         = {2013},
}

One might describe this method as having a $\Hilb^1$ flavour.
In fact, in light of \cite{lund} and \cite[Theorem 1]{rydh.nonsepd}, we do not believe our methods extend to non-separated algebraic spaces.\todo[color=yellow]{say that it is not clear whether gabriel should hold?}


add in gaitsgory section? \todo[inline,color=yellow]{add here gaigtsgory Lemma 4 and Prop 5?}
